ConvoFusion: Multi-Modal Conversational Diffusion for Co-Speech Gesture Synthesis

Gestures play a key role in human communication. Recent methods for co-speech gesture generation, while managing to generate beat-aligned motions, struggle generating gestures that are semantically aligned with the utterance. Compared to beat gestures that align naturally to the audio signal, semantically coherent gestures require modeling the complex interactions between the language and human motion, and can be controlled by focusing on certain words. Therefore, we present ConvoFusion, a diffusion-based approach for multi-modal gesture synthesis, which can not only generate gestures based on multi-modal speech inputs, but can also facilitate controllability in gesture synthesis. Our method proposes two guidance objectives that allow the users to modulate the impact of different conditioning modalities (e.g. audio vs text) as well as to choose certain words to be emphasized during gesturing. Our method is versatile in that it can be trained either for generating monologue gestures or even the conversational gestures. To further advance the research on multi-party interactive gestures, the DnD Group Gesture dataset is released, which contains 6 hours of gesture data showing 5 people interacting with one another. We compare our method with several recent works and demonstrate effectiveness of our method on a variety of tasks. We urge the reader to watch our supplementary video at our website.

==> Sections/X_suppl_CR.tex <==
\clearpage
\setcounter{page}{1}
\maketitlesupplementary
% 
% 
This supplementary document provides a glossary of notations used for method explanation in~\cref{supp:glossary} and discusses dataset statistics in~\cref{supp:datastats}. It also provides further details and analyses of word-excitation guidance in~\cref{supp:weg}, user study in~\cref{supp:userstudy} and implementation details in~\cref{supp:implement}. Moreover, we discuss evaluation metrics in~\cref{supp:metrics} and training details for baseline methods in~\cref{supp:baselines}.
% 
\section{Glossary for Notations}
% 
\label{supp:glossary}
% 
In~\cref{tab:supp-vars}, we provide a list of variables used in our the method and implementation details (Method Sec. and~\cref{supp:implement}) for ease of reference.
% 

\begin{table}[h]
    \centering
    \begin{tabular}{|c|c|} \hline 
         \textbf{Variable}& \textbf{Description}\\ \hline 
         $\mathbf{x}$& Gesture Sequence\\ \hline 
 $\mathbf{x}_b$, $\mathbf{x}_h$&Body and Hand Motions\\ \hline 
         $\mathbf{C}$& Conditioning Set\\ \hline 
         $\mathbf{z}$& Latent representation\\ \hline 
         $\mathbf{z}_b$, $\mathbf{z}_h$& Latent Representation for body and hands\\\hline
 $\xi_b$, $\xi_h$&Encoder for body and hands\\\hline
 $\mathcal{D}_b$, $\mathcal{D}_h$&Decoder for body and hands\\\hline
 ${\mathbf{x}^{\prime}}_b$, ${\mathbf{x}^{\prime}}_h$&Reconstructed motion for body and hands\\\hline
 $\mathbf{\hat{z}}$&Time-aware Latent Representation\\\hline
 $\epsilon_\theta$&Predicted noise\\\hline
 $f_\theta$&Denoiser neural network\\\hline
 $\mathbf{a}$&Audio Signal\\\hline
 $\boldsymbol{\tau}$&Text Embedding\\\hline
 $\boldsymbol{\tau}^{\prime}$&Text Embedding for co-participant\\\hline
 $\mathbf{s}$&Speaker Identity Token\\\hline
 $\mathbf{m}$&Active/Passive Bits for Latent Chunks\\\hline
 $w_c$&Modality guidance scale for condition $\mathbf{c}$\\\hline
 $S$&Number of tokens selected for WEG\\\hline
 $G_{exc}$&Word Excitation Guidance objective\\\hline
 $\mathbf{\tilde{z}^{(t)}}$&Updated latent after WEG\\\hline
    \end{tabular}
    \caption{\textbf{List of variables and their corresponding explanation}}
    \label{tab:supp-vars}
\end{table}
% 
\section{Dataset Statistics \& Discussion}
% 
\label{supp:datastats}
% 
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/dataset-aerial.png}
    \caption{Here, we show an over-arching view of our data-recording setup, where we have five people interacting with each other, while their motion tracking is recorded via a state-of-the-art marker-less motion capture system. Each person also has individual microphones which feed into our audio setup.}
    \label{fig:dataset-aerial}
\end{figure}
% 
% 
The proposed \dataset consists of $6$ hours of mocap data comprising of $5$ persons in the scene.
%
In total, we have 2.7M poses along with synchronized, per-person audio tracks and text transcripts (see~\cref{fig:dataset-aerial}).
%
The proposed dataset addresses a different aspect of human gestures, \textit{i.e.} group conversations, which is a sparsely researched setting.
%
This makes our dataset complementary to the existing monadic gesture datasets like BEAT.
%
We discuss how BEAT can be used with our framework along with our dataset in~\cref{ssec:baseline-train}.
% 
\par
% 
Finding a capture setting that elicits high density of meaningful, semantic gestures is indeed a challenging task.
%
These considerations lead us to capture the participants in a role-playing setting as they need to describe an imaginary world to each other, thereby leading to a high density of semantic gestures.
%
The setting also offers a clear intrinsic reward to the participants (of winning the game).
%
As we show in the video and~\href{https://vcai.mpi-inf.mpg.de/projects/ConvoFusion/}{website}, the gestures in our dataset are similar to the ones appearing in daily conversation because participants are simply discussing a game plan or their next steps in certain situations using language that is colloquially used in conversations. 
% 
Interestingly, the most relevant gestures to the game setting are pointing gestures (participants usually point to objects on table) which are considered deictic gestures, which happen frequently in normal conversations.
% 
We highlight that the proposed dataset is recorded in a markerless motion capture setup which it keeps the group conversation natural without restrictions of a capture suite or markers, thereby reducing the Observer's Paradox.
% 
Finally, the subjects are familiar with each other (esp. in the DnD setting) which further helps in more natural conversations.
% 
\begin{figure*}
    \centering
    \includegraphics[width=0.8\linewidth]{figures/WEG.pdf}
    \caption{\textbf{Algorithm overview of Word Excitation Guidance.}}
    \label{fig:word2joints}
\end{figure*}
% 
\section{On Word Excitation Guidance}
\label{supp:weg}
% 
In the following sections, we provide details of algorithm for word-excitation guidance and then perform additional in-depth analysis on its results.
% 
\subsection{Algorithm Details}
% 
% 
\begin{algorithm}
 \caption{Word-Excitation Guidance}
 \begin{algorithmic}[1]
 \renewcommand{\algorithmicrequire}{\textbf{Input:}}
 \renewcommand{\algorithmicensure}{\textbf{Output:}}
 \Require Set of tokens $\{\boldsymbol{\tau}_i\}_{i=1}^{S}$ \\ 
          Trained Diffusion Model $f_\theta$ \\
          Text Prompt $\boldsymbol{\tau} \in \mathbf{C}$, \\
          Diffusion Timesteps $T$ \\
          Step size $\alpha$
          % Softmax $\sigma$
 \Ensure  Denoised Latent $\mathbf{\hat{z}}^{(0)}$
 \\ \textit{Initialize} $\mathbf{\hat{z}}^{(T)} \sim \mathcal{N}(0, \mathbf{I})$ 
 % \\ \textit{Denoising Loop}
  \For {$t = T~to~0$} 
      \State $\_, A = f_\theta(\mathbf{\hat{z}}^{(t)}, t, \{\boldsymbol{\tau}\})$ \Comment{get attention for text}
      \State $A \leftarrow \operatorname{Softmax}(A_{\text{start}:\text{end}})$ \Comment{remove start/end of text}
      \State $A \leftarrow \operatorname{Gaussian}(A)$ \Comment{smooth out attentions}
      \State $G_{\mathrm{exc}} = \frac{1}{S} \sum_{i=1}^{S} (1 - \operatorname{max}(A_i))$ \Comment{calculate loss}
i      \State $\mathbf{\Tilde{z}}^{(t)} \leftarrow \mathbf{\hat{z}}^{(t)} - \alpha \cdot \nabla_{\mathbf{\hat{z}}^{(t)}}G_{\mathrm{exc}}$ \Comment{update latent}
      \State \textit{Perform Iterative refinement}~\cite{chefer2023attendexcite}
      \State $\epsilon_{\theta}^{(t)}, \_ = f_{\theta}(\mathbf{\Tilde{z}}^{(t)}, t, \mathbf{C})$ \Comment{estimate noise}
      \State \textit{Perform Modality Guidance}
      \State $\mathbf{\hat{z}}^{(t-1)} \leftarrow \operatorname{SchedulerStep}(\mathbf{\Tilde{z}}^{(t)}, \epsilon_{\theta}^{(t)})$
  \EndFor \\
 \Return  $\mathbf{\hat{z}}^{(0)}$ 
 \end{algorithmic} 
 \label{algo:semantic}
 \end{algorithm}
% 
% 
% \par
% 
The process of word-excitation guidance involves modifying the usual denoising loop by updating the latents at each timestep.
% 
Before updating the latents, we normalize the attention maps by removing attention on the start and end tokens because each training batch contains text prompts of different lengths.
% 
Moreover, we observe that our latent diffusion framework assigns high attention to the start token in text (shown in Figure~\ref{fig:attmaps}), therefore, we mitigate this issue by considering the attention on the actual text tokens.
% 
Then we apply Gaussian smoothing over the remaining attention map for stable generation results without any jerks in motion.
% 
This ensures flexibility to focus on a neighbourhood of words instead of one word by avoiding gradient updates at only the chosen tokens ignoring its neighbourhood.
% 
Next, we calculate the average for the loss over all the \textit{focus} tokens to equally transfer gradients for all the focused words.
% 
Note that, this is different from image-based semantic guidance~\cite{chefer2023attendexcite}, where Chefer~\etal apply smoothing on attention for only the chosen words/tokens which ignores the neighbourhood tokens. 
% 
Moreover, their loss aggregation only enables gradient transfer for tokens with the lowest attention instead of all focused tokens by using a $\operatorname{max}$ function instead of $\operatorname{mean}$ like us.
% 
% 
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/vertical-heatmap.pdf}
    \caption{Heatmap showing the distribution of velocity of all joints compared with motion-aligned text (focused words are highlighted in red). We see high joint velocity for hand and arm joints around the words ``french'' and ``now''.}
    \label{fig:word2joints}
\end{figure}
% 
The complete process is presented in Algorithm~\ref{algo:semantic}.
% 
\subsection{Additional Analysis}
% 
\noindent
\textbf{Joints Affected Per Word.}
% 
Recall that word-level excitation guidance steers the gesture generation process through the denoising network to have pronounced gestures at certain words in the text. 
% 
It gives a fine mechanism for semantic control over gesture generation. In~\cref{fig:word2joints}, we present an analysis of how this mechanism affects each joint in the generation. The figure encodes as heatmap the velocity of each joint in response to the text tokens; the assumption being that high velocity implies heavier gesturing. We see that the hand and the arm joints are affected the most at the focused words. Interestingly, minimal attention is focused on the lower body; this is expected as most gestures are predominantly upper-body motions.
% 
\par
\noindent
\textbf{Choice Of Words.} 
% 
Specific types of gestures tend to correlate with certain linguistic structures and parts of speech.
%
Thus, for analysis, we conduct experiments with attention focused on these elements. 
% 
To extract phrases that may map onto a semantic gesture, we select \textit{random} three-word phrases in the text. 
% 
% 
To experiment with individual words, we can focus on nouns and verbs as they have a higher chance of mapping onto \textit{iconic} gestures. 
%
Adverbs and adjectives can also be chosen since they can convey spatiotemporal properties of events and entities.
% 
% 
This choice mechanism, which is motivated by the mapping of gestures to linguistic structures, is also flexible enough for the users to choose different linguistic features to focus on. 
%
We also consider optimal stress word discovery as a future endeavour.
% 
% 
Lastly, the success of word-level semantic guidance is also affected by the amount of stress certain word has in the audio.
% 
We show attention results for phrases and words in~\cref{fig:attmaps} and gesture generation results in supplementary video.
%
\par
\noindent
\textbf{Interpreting Word-Excitation through Attention Maps.}
Since we perform word-level guidance on text attention maps, we include example results in~\cref{fig:attmaps}.
% 
The attention map $A$ is dependent on text conditioning and diffusion timestep and shows the relation between chunks of latent representation and text tokens.
% 
Therefore, performing word-level guidance at each diffusion timestep yields slightly different attention distribution over words.
% 
We observe that as we move from $t=T$ to $0$, focused word tokens (highlighted in red) start to get high attention, especially after $t=T/2$.
% 
We also see the effect of Gaussian smoothing as the attention on focus words is not sharply focused on only those words.
% 
Rather it is spread over its neighbouring tokens as well.
% 
Lastly, notice the striped pattern of the attention weights. 
%
This arrangement is a manifestation of the separated body and hand latents that have been stacked alternatively.
% 
It shows that the network learns to perform attention in a separate manner for both types of latents and guidance affects them differently across different layers as well.
% 
% 
\begin{figure*}
% 
\begin{subfigure}[h]{0.98\textwidth}
\includegraphics[width=\linewidth]{figures/att_maps/b_990.jpg}
\caption{Text: ``and dried \textcolor{red}{fruits in september} you're boiling it in''} \label{fig:attmap-b990}
\end{subfigure}
\hfill
\begin{subfigure}[h]{0.98\textwidth}
\includegraphics[width=\linewidth]{figures/att_maps/b_400.jpg}
\caption{Text: ``and dried \textcolor{red}{fruits in september} you're boiling it in''} \label{fig:attmap-b400}
\end{subfigure}%
\hfill
\begin{subfigure}[h]{0.98\textwidth}
\includegraphics[width=\linewidth]{figures/att_maps/b_10.jpg}
\caption{Text: ``and dried \textcolor{red}{fruits in september} you're boiling it in''} \label{fig:attmap-b10}
\end{subfigure}
% 
\begin{subfigure}[h]{0.98\textwidth}
\includegraphics[width=\linewidth]{figures/att_maps/c_990.jpg}
\caption{Text: ``\textcolor{red}{after} a \textcolor{red}{while came} and settled''} \label{fig:attmap-c990}
\end{subfigure}
\hfill
\begin{subfigure}[h]{0.98\textwidth}
\includegraphics[width=\linewidth]{figures/att_maps/c_400.jpg}
\caption{Text: ``\textcolor{red}{after} a \textcolor{red}{while came} and settled''} \label{fig:attmap-c400}
\end{subfigure}%
\hfill
\begin{subfigure}[h]{0.98\textwidth}
\includegraphics[width=\linewidth]{figures/att_maps/c_10.jpg}
\caption{Text: ``\textcolor{red}{after} a \textcolor{red}{while came} and settled''} \label{fig:attmap-c10}
\end{subfigure}
% 
% 
\caption{\textbf{Text attention example with focus on a phrase: (a) $t=990$ (b)  $t=400$ (c) $t=10$ and example with multiple individual words: (d) $t=990$ (e)  $t=400$ (f) $t=10$.} Vertical axes show $M \times 2$ latent chunks where even and odd indices stand for body and hand joints respectively. Horizontal axes show word tokens where focused words are highlighted in red. Attention changes are highlighted in red boxes where neighboring tokens are also included to show the effect of Gaussian smoothing. Lastly, ``\textless bos\textgreater'' \& ``\textless eos\textgreater'' tokens represent start and end of the text (refer~to Method Sec.}
\label{fig:attmaps}
\end{figure*}
% 
\par
\noindent
\textbf{Limitations.}
% 
% 
Our method is, after all, a data-driven method.
%
It depends on the learned conditional gesture distribution of text and other modalities, which can lead to it generating the most common gesture type (\textit{beat gestures}) seen for some words.
% 
Consequently, performing word-level guidance does not always guarantee the specific motion of accurate semantic sub-gesture type (\textit{iconic, deictic, metaphoric etc.}) at the focused word or phrase.
% 
However, as we analyzed, the usage of word-excitation guidance (WEG) mostly results in a semantically meaningful gesture as compared to the base prediction without WEG.
% 
For future works, a more explicit representation of gesture types and their mapping to words can be provided as a conditioning, which might help in predicting semantically accurate gestures.
% 
Secondly, the amount of focus each word/phrase attains in terms of gesture movements is dependent on the fact that speech also contains certain prosodic stress for that word. 
% 
%
% 
Similarly, if the gestures around focused words are already stressed adequately in motion or those words already have high attention on them, then the change introduced by guidance will only be subtle.
% 
Lastly, the choice of words affects the type of stress in gesture movements predicted and this can be highly subjective. 
% 
\section{User Study}
\label{supp:userstudy}
% 
For evaluation of monadic synthesis, the user were shown a randomly sampled set of $10$ forced-choice questions.
%
Each question included a side-by-side animation of our method along with one of MLD~\cite{mld}, CaMN~\cite{liu2022beat}, or the ground-truth.
%
The participants had to answer two question, (a) \textit{``Which of the two gesture motions appears more natural?} and (b) \textit{``Which of the two gesture motions corresponds better with the spoken utterance?''}. 
%
These questions try to gauge plausibility of the motions and alignment of the generated gestures with the utterance.
% 
For the task of dyadic synthesis, we showed $5$ randomly sampled forced choice questions to each participant, comparing our method with the adapted MLD and the ground-truth.
% 
The participants had to judge the naturalness of the motions similar to previous task and also answer the question: \textit{``In which of the two interactions, the motion of interacting character fits well with both speech of the the main agent as well as their own speech, if any.''}
% 
We report percentage preference for both tasks.
% 
In the third section, we asked the users to evaluate the word-excitation guidance.
%
Each question included three motions---corresponding to the ground-truth motion, non-guided motion, and word-excitation guided motion --- as well as the words that need to be excited during synthesis.
% 
We compare ground-truth, non-guided gesture, and word-excitation guided gesture.
%
The users were asked to rate each motion on a Likert scale of $1$-$5$, with $5$ indicating the most semantically aligned gesture.
% 
\section{Implementation Details}
\label{supp:implement}
\textbf{Motion Representation.} 
% 
The motion $\mathbf{x}$ corresponds to the root-relative 3D coordinates for all $J-1$ joints and camera-relative translation of the root joint. 
% 
The hand joints are also made relative to their corresponding wrist joint.
% 
We also pre-process the joint positions following~\cite{humanml3d} by normalizing the motion sequence to start the root trajectory from the origin while facing the positive z-axis.
% 
% 
\paragraph{VAE.}
% 
We implement decoupled scale-aware VAE using two transformer encoders in order to make two halves of the latent representation focus separately on body and hands. 
% 
Each encoder is based on transformer architecture with long skip-connections utilized by Chen \etal~\cite{mld} as they prove this method to be effective in retaining high information density in latent representation.
% 
% 
The output of each encoder is combined into two quantities to represent Gaussian distribution parameters $\boldsymbol{\mu}_\phi$ and $\mathbf{\Sigma}_\phi$ of the combined scale-aware latent space $\mathcal{Z}$, where $\phi$ represent learnable weights of encoders.
% 
We can sample $\mathbf{z}^{2 \times d}$ using reparameterization trick~\cite{vae}.
% 
\par
We train the VAE until convergence with a combination of losses to achieve the desired reconstruction quality.
% 
MSE-based reconstuction loss is applied on the reconstructed motion $\mathbf{\hat{x}}$:
% 
\begin{equation}
    \mathcal{L}_2 = \norm{\hat{\mathbf{x}} - \mathbf{x}}_2
\end{equation}
% 
Moreover, Kullback-Liebler divergence $\mathcal{L}_{KL}$ is used for regularizing the latent space:
% 
\begin{equation}
    \mathcal{L}_{KL} = D_{KL}( \mathcal{N}(\mathbf{z};\boldsymbol{\mu}_\phi, \mathbf{\Sigma}_\phi) || \mathcal{N}(\mathbf{z};0, \mathbf{I}))
\end{equation}
% 
We also apply Bone Length Consistency Loss~\cite{mofusion}, which ensures that bone lengths do not vary across frames in a gesture sequence by minimizing the variance of bone lengths $l_n$.
% 
\begin{equation}
    \mathcal{L}_{bone} = \frac{\sum_{n=1}^N (l_n - \bar{l})^2}{n-1}, 
\end{equation}
% 
Lastly, the VAE loss also contains a Laplacian regularization term $\mathcal{L}_{lap}$ as described earlier, to better reconstruct subtle jerks in gestures and reduce jitter. 
% 
\begin{equation}
    \mathcal{L}_{VAE} = \mathcal{L}_2 + \lambda_{KL} \mathcal{L}_{KL} + \lambda_{lap} \mathcal{L}_{lap} + \lambda_{bone} \mathcal{L}_{bone}
\end{equation}
% 
% 
\par
% 
In order to achieve time-aware latent representation, we encode time-aligned $M$ chunks of motion $\{\mathbf{{x}}_i^{\prime}\}_{i=1}^{M}$ using encoders by passing each $\mathbf{{x}}_i^{\prime}$ from $\xi_b$ and $\xi_h$ to get $\mathbf{\hat{z}}_i$. 
% 
This sequence $\mathbf{\hat{z}} = \{\mathbf{\hat{z}}_i\}_{i=1}^M$ is applied with a positional encoding~\cite{vaswani2017posenc} along $M$ to represent time-alignment.
% 
Along with positional encoding as queries, $\mathbf{\hat{z}}$ passed onto decoder $\mathcal{D}$ as a memory to obtain $\mathbf{\hat{x}}$.
% 
% 
% 
This unique structure of $\mathbf{\hat{z}}$ allows us to perform arbitrary length generation with latent diffusion models, which generally are constrained to due to fixed-length generation. 
\begin{table}[]
    \centering
    \begin{tabular}{|c|c|} \hline  
         \textbf{Hyperparameter}&  \textbf{Value}\\ \hline  
         Latent dimension $d$& 
    128\\ \hline  
 Motion Length $N$&128\\ \hline  
 Number of Joints $J$&63\\ \hline  
 Motion chunks $M$ &8\\ \hline  
 $\lambda_{KL}$&0.05\\ \hline  
 $ \lambda_{lap}$&1\\ \hline
 $\lambda_{bone}$&1\\ \hline  
 Transformer Layers&5\\\hline
 Attention Heads&2\\\hline
 Learning Rate&$1\e{-4}$\\\hline
 Optimizer&AdamW~\cite{adamw}\\\hline
 FPS&25\\\hline \end{tabular}
    \caption{List of values used for training VAE for our method}
    \label{tab:vae_hyperparam}
\end{table}
% 
% 
\paragraph{Perpetual Generation Rollout.}
% 
\begin{figure}
    \centering    
    \includegraphics[width=\columnwidth]{figures/inpainting2.pdf}
    \caption{\textbf{Iterative process for the perpetual rollout of arbitrary-length generation.} This is based on the diffusion inpainting technique.}
    \label{fig:inpaint}
\end{figure}
% 
During inference of our diffusion framework, we leverage the time-aware latent sequence $\{\mathbf{\hat{z}}_i\}_{i=1}^M$ to autoregressively generate latent sequences for arbitrarily long sequences.
% 
As compared to earlier approaches \cite{liu2022beat, rnn_based3}, we do not concatenate our model's output which may cause irregular motion at the point of joining. 
% 
We also do not encode variable length sequences in our VAE framework as done by MLD~\cite{mld}.
% 
Instead, we propose an autoregressive generation approach to predict the time-aware latent sequence beyond $M$ number of chunks. 
% \
The key to this approach is an iterative process (shown by~\cref{fig:inpaint}) where a sequence of future latent chunks is predicted based on the last $k$ current latent chunks through a denoising process.
%
Given the sequence $\mathbf{\hat{z}} \in \mathbb{R}^{M \times 2 \times d}$ represents motion $\mathbf{x}$ of first $N$ frames, we call it $\mathbf{\hat{z}}_{1:M}$ which is known to us.
%
We utilize the last $k$ latent chunks from this known sub-sequence, i.e. $\mathbf{\hat{z}}_{(M-k):M}$, and generate the next $M-k$ latent chunks through the denoising process to obtain a new overlapping sequence $\mathbf{\hat{z}}_{(M-k):(2M-k)}$. 
%
Every time we need to generate the next $(M-k):(2M-k)$ sequence, we first inject noise to the previously known $(M-k):M$ sub-sequence until the $t-1$ diffusion timestep. 
% 
Then, this sub-sequence is concatenated with the latent sub-sequence at $M:(2M-k)$ which contains new latents for the non-overlapping part in $(M-k):(2M-k)$ sequence.
% 
This concatenated sequence $\mathbf{\hat{z}}^{(t-1)}_{(M-k):(2M-k)}$ is then passed to the next denoising iteration where the process repeats by noising the known part for the next diffusion timestep.
% 
This technique follows the masked denoising technique used for diffusion image inpainting \cite{lugmayr2022diffinpaint}.
%
\begin{equation}
	\mathbf{\hat{z}}^{(t-1)}_{M-k:2M-k} = \oplus(q(\mathbf{\hat{z}}_{M-k:M}, t-1), \mathbf{\hat{z}}^{(t-1)}_{M:2M-k})
\end{equation}
%
Here, the $\oplus$ operator concatenates along latent chunks to total length of $M$ for each sequence.
%
When applied iteratively to the subsequent new frames, this process enables an autoregressive rollout of fixed-length gesture sequences into infinite-length synthesis. 
% %
We set the value of the hyperparameter $k$ as $k=M/2$ for simplicity.
%
% 
% 
% 
% 
\paragraph{Details on Denoising Network.}
% 
% 
We design denoising network for the latent diffusion framework to predict $\epsilon_{\theta}(\mathbf{\hat{z}}^{(t)}, t)$. 
% 
We implement the denoising schedule based on DDPM framework with hyperparameters presented in~\cref{tab:diff_hyperparam}.
%
This framework consists of a Markovian chain of successively adding Gaussian noise $\epsilon$ to $\mathbf{\hat{z}}^{(0)}$ for $T$ timesteps i.e. \textit{forward diffusion} process.
%
Through this process, $\mathbf{\hat{z}}^{(0)}$, which was sampled from data distribution, becomes $\mathbf{\hat{z}}^{(T)}$, which follows noise distribution $\mathcal{N}(0, \mathbf{I})$ assuming $T$ is sufficiently large.
% %
\begin{equation}
	q \big(\mathbf{\hat{z}}^{(1:T)} | \mathbf{\hat{z}}^{(0)} \big) = \prod_{t=1}^{t=T} q\big(\mathbf{\hat{z}}^{(t)} | \mathbf{\hat{z}}^{(t-1)}\big)
\end{equation}
% %
where $q(\mathbf{\hat{z}}^{(t)} | \mathbf{\hat{z}}^{(t-1)}) = \mathcal{N}(\mathbf{\hat{z}}^{(t)}|\sqrt{1-\beta_t}\mathbf{\hat{z}}^{(t-1)}, \beta_t \mathbf{I})$, describes evolution of latent distribution during the noising process at time step $t$.
% % 
Here, $\beta_t$ represents the rate of diffusion. 
%
%
The \textit{reverse diffusion} process consists of denoising $\mathbf{\hat{z}}^{(T)} \sim \mathcal{N}(0, \mathbf{I})$ for $T$ timesteps to generate a latent sequence $\mathbf{\hat{z}}^{(0)}$:
% 
\begin{equation}
p_\theta\big(\mathbf{\hat{z}}^{(0:T)}\big) = p\big(\mathbf{\hat{z}}^{(T)}\big) \prod_{t=1}^T p_\theta\big(\mathbf{\hat{z}}^{(t-1)} | \mathbf{\hat{z}}^{(t)}\big),    
\end{equation}
% 
where $p_\theta(\mathbf{\hat{z}}^{(t-1)} |\mathbf{\hat{z}}^{(t)})$ is approximated using a denoiser neural network~$f_{\theta}(\mathbf{\hat{z}}^{(t-1)} | \mathbf{\hat{z}}^{(t)}, t, \mathbf{C})$, which is trained to predict noise
% 
We use transformer decoder network as $f_{\theta}$ which takes $\mathbf{\hat{z}}^{(t-1)}$ as queries along with diffusion timestep $t$ and conditioning set $\mathbf{C}$ as memory input.
% 
We apply positional encoding to queries and individual memory inputs similar to~\cite{vaswani2017posenc}.
% 
To better distinguish between body and hand latents in $\mathbf{\hat{z}}^{(t-1)}$, we add a learned embedding that aims to differentiate between body and hand parts of the latent representation.
% 
We also add a learned embedding to each element of our conditioning set $\mathbf{C}$ separately which helps the network differentiate between different conditioning types.
%
Each transformer layer starts with Self-Attention and LayerNorm layers, along with a time-layer based on Stylization Block~\cite{motiondiffuse} to incorporate diffusion timestep embedding.
% 
Multi-modal cross attention consists of the same number of heads as the number of elements in the conditioning set $\mathbf{C}$.
% 
The outputs of all heads are aggregated using a linear projection, which is followed by another linear layer with GeLU activation~\cite{gelu}.
% 
% 
\begin{table}[]
    \centering
    \begin{tabular}{|c|c|} \hline  
         \textbf{Hyperparameter}&  \textbf{Value}\\ \hline  
         $d$& 
    128\\ \hline  
 Range of $\beta_t$& $[8.5\e{-4},1.2\e{-2}]$\\ \hline  
 $T$&1000\\ \hline  
 $\beta_t$ Schedule&Scaled Linear~\cite{ldm}\\ \hline  
 Self-Attention Heads&4\\ \hline  
 Decoder Layers&9\\ \hline
 Learning Rate&$7\e{-5}$\\\hline
 Optimizer&AdamW\\\hline \end{tabular}
    % 
    \caption{List of hyperparameters for denoising network in our method}
    % 
    \label{tab:diff_hyperparam}
\end{table}
% 
\par
\noindent
\textbf{Guidance Parameters.}
% 
% 
We modify classifier-free guidance to add modality-level control for each element in our conditioning set. The random modality dropout rate is set to 10\% and global guidance scale $\lambda_m$ is set to 7.5.
% 
The values of $w_c$ is determined by the task at hand.
% 
For example, if we want to extract only the gesture styles of different speakers regardless of input text and audio, we set all $w_c$ to 0 except $w_{\mathbf{s}} = 1$, which corresponds to speaker identity.
% 
This will generate \textit{unconditional} gestures in the style of a specific speaker (see supplemental video for the example).
% 
For word-excitation guidance, step size $\alpha$, goes from 100 to 70.71 as it varies w.r.t. diffusion timestep.
% 
The kernel size for Gaussian smoothing is 3.
% 
% 
% 
% 
\par
\noindent
\textbf{Semantic Consistency Evaluation Model:}
%
Our method can generate semantically meaningful gestures (as shown in Suppl. Video), thanks to the proposed Word Excitation Guidance (WEG).
% 
%
% 
We conduct this ablation the following way.
%
First, we trained a binary classifier that classifies $1$s motions of the BEAT dataset into either beat gesture, or semantic gesture type (based on the GT labels).
% 
Here semantic class consists of \textit{iconic}, \textit{metaphoric}, and \textit{deictic} classes.
%
% 
% 
%
This classifier is then used as an oracle to compute the recall of our generated motions for semantic class predictions.
%
Specifically, we extract the speech and text for the sentence in which a semantic gesture has been labeled in dataset.
%
These are then input to \model to generate the corresponding gestures, with and without WEG.
%
For the case of WEG, we focus on the exact words wherein the semantic gesture occurs in the sentence.
% 
% 
% 
% 
\section{Evaluation Metrics}
\label{supp:metrics}
% 
We report quantitative results on Beat Alignment Score~\cite{aichoreo}, FID, Diversity, L1 Divergence and Semantic Relevance Gesture Recall (SRGR)~\cite{liu2022beat} and here we briefly describe each one of them.
% 
Beat Alignment Score was initially introduced~\cite{aichoreo} to measure the alignment of music beats to dance motion for the task of music-to-dance synthesis. 
% 
This has also been adapted for the task of gesture synthesis, where it measures the correlation between gesture beats and audio beats. 
% 
It is useful in differentiating between static motions which do not align well with the audio from natural-looking gestures which have speech-aligned kinematic beats.
% 
However, it can report false high values if the motion has a large amount of jitter because it would assume beats created by jitter align well with most of the audio beats.
% 
We can see this happening for methods that show high jitter~\cite{rnn_based3, diffgesture} in our experiments. 
% 
They have high Beat Alignment score while their FID is also large. 
% 
\par
% 
We employ the Frechet Inception Distance (FID) metric provided by Yoon \etal~\cite{rnn_based3}, also known as FGD.
% 
We trained our FID network using implementation by Liu~\etal~\cite{liu2022beat}.
% 
It is based on an autoencoder network that is trained for reconstruction task, and is calculated by comparing features of the ground truth data $\mathbf{x}$ and generated data $\mathbf{\hat{x}}$ through:
% 
\par
\footnotesize
\begin{equation}
    \operatorname{FGD}(\mathbf{x}, \mathbf{\hat{x}}) = \norm{\mu_r - \mu_g}^2 + \operatorname{Tr}(\Sigma_r + \Sigma_g - 2 \sqrt{\Sigma_r \Sigma_g} )
\end{equation}
\normalsize
% 
Methods that generate diverse gestures like ours and do not contain pre-pose information unlike CaMN~\cite{liu2022beat} and MultiContext~\cite{rnn_based3}, may suffer on this metric because our gestures will not try to match ground truth motion. 
% 
Diversity computes the average pairwise Euclidean distance of the gesture generations in the test set.
% 
L1 Divergence (also called L1 variance) measures the distance of all frames $N$ in a gesture sequence from their mean $\mu_N$. 
% 
Here $B$ is size of test set.
% 
\begin{equation}
    \operatorname{L1div}(\mathbf{x}) = \frac{1}{B} \sum_{i=1}^N |\mathbf{x}_i - \mu_N|
\end{equation}
% 
This metric specifically identifies if the gestures are static in movement and make less diverse movements along the generation length.
% 
As shown in supplemental video, CaMN~\cite{liu2022beat} and MLD~\cite{mld} suffer from this problem whereas, our method predicts different gestures according to the text and audio conditionings and does not have static motion.
% 
\par
% 
Semantic Relevance Gesture Recall (SRGR) uses semantic score labelled in BEAT~\cite{liu2022beat} as a weight for the Probability of Correct Keypoint (PCK) between the generated gestures and ground truth gestures. It aims to reward being close to ground truth motion at points where a semantically relevant gesture exists while also predicting diverse gestures, as mentioned by Liu \etal~\cite{liu2022beat}.
% 
This metric has a similar issue as FID as it compares PCK between ground truth and prediction and due to many-to-many correspondence between gestures and speech, this might not be suitable. 
% 
% 
Therefore, we conclude that each metric focuses on certain aspects of gesture generation and human-annotated user study results are more conclusive to determine better generation quality and to perform a holistic analysis of gesture quality
% 
% 
\section{Baseline Training Details}
\label{supp:baselines}
% 
In the following, we provide details on how we process all the different modalities for our dataset (\cref{ssec:baseline-datasets}) and provide details for training each method we use for comparison (\cref{ssec:baseline-train}).
% 
% 
\subsection{Dataset}
\label{ssec:baseline-datasets}
% 
\par
\noindent
\textbf{BEAT.} 
%
We utilize the BEAT dataset~\cite{liu2022beat} in order to augment the training data for our method so that it better generalizes to the task of monadic gesture synthesis.
% 
It consists of 60 hours of English speaking training data, spanning 30 subjects that perform gesture motions.
% 
The dataset is rich in good training examples for monologue setting which can serve as a good baseline dataset to train our method.
% 
Inherently, BEAT's motion representation is different than what we use to train our method.
% 
Therefore, we re-target their skeleton definition to our skeleton definition in order to match it with our \dataset dataset.
% 
Moreover, we convert their representation from BVH-based euler angle representation to joint positions using forward kinematics.
% 
Then we resample their dataset from 120 FPS to 25 FPS in order to match it with our training configuration. 
%
Lastly, we apply the preprocessing steps mentioned in~\cref{supp:implement} to get the final motions which we separate into 5.12-sec chunks i.e. 128 frames for training our method.
% 
\par
\noindent
\textbf{\dataset.}
% 
To apply our method to the task of dyadic synthesis, we utilize our recorded \dataset dataset (see~\cref{fig:dataset-aerial}) to extract interactions between people in our dataset. 
% 
We record the dataset in BVH format as well, however, we extract joint positions for training our method.
% 
We standardize dataset FPS to 25.
% 
Each of the five people in our dataset has their own separate audio channel which we have post-processed to get clean and denoised audio.
% 
We align audio channels with the recorded tracking and verify it manually as well. 
% 
Finally, we separate out motions for each person and assign them identities which are kept consistent across multiple recording sessions.
% 
Then, we preprocess the dataset and separate it out in chunks of 128 frames.
% 
\par
\noindent
\textbf{Training/Test Splits.}
% 
We split the BEAT dataset by reserving 5 out of 30 English speakers for the testing set, while the remaining go into training and validation splits.
% 
Therefore, all the results and comparisons on monadic synthesis using BEAT dataset are provided on unseen speakers which shows a method's generalizability to unseen audio and text inputs.
% 
For dyadic synthesis, we randomly sample and take out 10 percent for testing and rest for training and validation.
% 
\par
\noindent
\textbf{Representation of Modalities.}
% 
We process audio by sampling it to 16000 Hz and extracting melspectrograms using librosa toolbox~\cite{librosa}.
% 
We use 80 mel-bands and a hop length of 512 for melspectrogram conversion.
% 
We process text through text tokenizer and convert them to embeddings through T5 text encoder~\cite{raffel2020t5} implementation by Hugging Face~\cite{wolf-etal-2020-transformers}.
% 
% 
\par
Lastly, all methods are trained on these dataset splits to ensure fairness. There are some differences between the type of representation used for audio and text in each method, which we elaborate on in the next section.
% 
% 
\subsection{Methods for Comparison}
\label{ssec:baseline-train}

\par
\textbf{ConvoFusion (Ours).}
% 
We train our method on 128-frame sequences by learning a latent space representation of them
% 
Then we use our diffusion framework on top of it.
% 
Interestingly, we can incorporate both monadic and dyadic gesture synthesis tasks into single training.
% 
Thanks to Modality Guidance, we can use different modalities interchangeably by dropping them out of the training batch and setting an unconditional token in their place.
% 
For example, BEAT dataset only contains single-person gesture annotations and does not contain a co-participant, hence making it non-trainable for the task of dyadic synthesis. 
% 
However, we can simply provide an unconditional token for the co-participant's text which automatically turns the contribution of the corresponding modality guidance term to zero, and BEAT dataset can be trained jointly with \dataset dataset.
% 
A similar approach can be taken for semantic annotation labels provided by BEAT dataset, which we do not provide for ours.
% 
% 
\par
\noindent
\textbf{CaMN~\cite{liu2022beat} \& Multi-Context~\cite{rnn_based3}.}
% 
We train both of these methods using the official implementation of CaMN by Liu~\etal on GitHub. 
% 
The only modification that took place was the addition of our dataset pipeline which includes our version of BEAT dataset and \dataset dataset, which makes the motion dimensions from 141 to 189 to match to our setting.
% 
We use the provided $\operatorname{WavEncoder}$ in the implementation to process audio signals instead of melspectrograms.
% 
Lastly, we use motion-aligned text instead of normal text inputs to be consistent with them.
% 
We also use the provided text-encoder to add our textual vocabulary to the text tokenizer for text preprocessing.
% 
\par
\noindent
\textbf{MLD~\cite{mld}.}
% 
This method by Chen~\etal which uses latent diffusion models, was presented for the task of text-to-motion synthesis. We extend this method for the gesture synthesis task by utilizing our training procedure.
% 
To be consistent with their method, we use the text encoder which was used by MLD.
% 
\par
\noindent
\textbf{DiffGesture~\cite{diffgesture}.}
% 
We use their official implementation on GitHub to train this method for the task of monadic gesture synthesis. 
% 
Since DiffuGesture~\cite{diffugesture} does not provide an implementation for dyadic synthesis task and it is highly based on DiffGesture, we follow DiffuGesture's implementation details as close as possible and adapt DiffGesture to the dyadic synthesis task.
% 
As this method was originally trained on TED Dataset~\cite{yoon19robots}, which contains only the upper body, we double the capacity of their transformer network to cater to the increase in dimensionality in our setting to ensure fairness.
% 
The audio and text processing is kept consistent with DiffGesture's implementation. 
% 
Lastly, for the task of dyadic synthesis, we provide co-participant's text as an additional conditioning input to match it with our training pipeline.
% 

==> rebuttal.tex <==
% \documentclass[10pt,twocolumn,letterpaper]{article}
% \usepackage[rebuttal]{cvpr}

% % Include other packages here, before hyperref.
% \usepackage{graphicx}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{booktabs}

% % Import additional packages in the preamble file, before hyperref
% \input{preamble}

% % If you comment hyperref and then uncomment it, you should delete
% % egpaper.aux before re-running latex.  (Or just hit 'q' on the first latex
% % run, let it finish, and you should be clear).
% \definecolor{cvprblue}{rgb}{0.21,0.49,0.74}
% \usepackage[pagebackref,breaklinks,colorlinks,citecolor=cvprblue]{hyperref}

% % Support for easy cross-referencing
% \usepackage[capitalize]{cleveref}
% \crefname{section}{Sec.}{Secs.}
% \Crefname{section}{Section}{Sections}
% \Crefname{table}{Table}{Tables}
% \crefname{table}{Tab.}{Tabs.}
% \input{macros.tex}
% % If you wish to avoid re-using figure, table, and equation numbers from
% % the main paper, please uncomment the following and change the numbers
% % appropriately.
% %\setcounter{figure}{2}
% %\setcounter{table}{1}
% %\setcounter{equation}{2}

% % If you wish to avoid re-using reference numbers from the main paper,
% % please uncomment the following and change the counter for `enumiv' to
% % the number of references you have in the main paper (here, 6).
% %\let\oldthebibliography=\thebibliography
% %\let\oldendthebibliography=\endthebibliography
% %\renewenvironment{thebibliography}[1]{%
% %     \oldthebibliography{#1}%
% %     \setcounter{enumiv}{6}%
% %}{\oldendthebibliography}

% \newcommand{\Rr}{\textbf{\textcolor{Orange}{R\_59mc}}}
% \newcommand{\Rb}{\textbf{\textcolor{YellowGreen}{R\_tZ8A}}}
% \newcommand{\Ra}{\textbf{\textcolor{ForestGreen}{R\_aN4a}}}


% %%%%%%%%% PAPER ID  - PLEASE UPDATE
% \def\paperID{4824} % *** Enter the Paper ID here
% \def\confName{CVPR}
% \def\confYear{2024}

% \begin{document}

% %%%%%%%%% TITLE - PLEASE UPDATE
% \title{ConvoFusion: Multi-Modal Conversational Diffusion for Co-Speech Gesture Synthesis \vspace{-1mm}}  % **** Enter the paper title here

% \maketitle
% \thispagestyle{empty}
% \appendix

% %%%%%%%%% BODY TEXT - ENTER YOUR RESPONSE BELOW
% We thank the reviewers for their feedback and are happy that they found that our work ``proposes many interesting ideas'' (\Ra), has  experimentally demonstrated the effectiveness of our method (\Ra, \Rr, \Rb), proposes a dataset that advances the research in multi-party gestures (\Rb) and addresses an interesting and significant task (\Rr).
% %
% % We are also delighted to hear the feedback that method has no major weaknesses (\Ra).
% % 
% %The typographical mistakes in text and equations will be corrected [\Ra, \Rr].
% % 
% We address the key concerns in detail. 
% \par
% \noindent \textbf{Novelty of chunk-wise embedding [\Rr]:}
% We thank the reviewer for pointing us to EmotionGesture~\cite{qi2024emotiongesture} (\textit{which we believe is not a peer-reviewed publication yet}).
% %
% We believe EmotionGesture utilizes chunkwise embeddings in a different manner.
% %
% Their motivation for operating in chunked motion space is to improve smoothness by adding additional temporal context (derived from the initial seed motion).
% %They propose to encode emotion-specific motion features as latent embeddings.
% %
% Our chunk-wise embeddings, on the other hand, are designed to enable perpetual motion rollout within a latent diffusion model framework (Ln266-275).
% % The key difference between our chunk-wise (or time-aware) latent representation and EmotionGesture (and other such latent-representation methods like T2M-GPT) is that we utilize these time-aware chunks to enable long-term generation in latent diffusion models. \RD{This is not a fair point. they don't, but \textit{can they}?}
% %
% %As we explain in Ln266-275, we require chunked embeddings to facilitate infinite gesture rollout.
% %
% %By encoding short (chunked) sequences of motion into latent vectors and then using a decoder that jointly decodes a sequence of such chunked embeddings, we ensure that the decoded motions are temporally consistent.
% %
% EmotionGesture is neither based on diffusion models nor decodes them jointly in a manner as we do, and requires seed motion which we don't.
% % 
% % We encode each chunk in the embedding using separate encoders and then decode all of the chunks together using one decoder, which is a different approach compared to what EmotionGesture does. 
% % 
% %
% % Our motivation for long-term generation is explained in Line 266-275 in Section 3.1 and the technical details are referred to in L283-285, 581-587 and in supplementary documents: L154-190.
% % 
% To the best of our knowledge, infinite rollout of motion generation using latent diffusion models has not been proposed in conjunction with transformer-based encoder-decoder architectures.% and our method contributes to that. 
% % 
% The main contribution of our method lies in \textit{controllable gesture synthesis} and \textit{generalization to monadic and dyadic settings} within a unified approach.
% \par
% \noindent \textbf{Disentangled representation is not novel [\Rr]:} 
% We \textit{do not} claim that the disentangled skeleton representation is the key contribution of the paper.
% %
% The key contribution of our work lies in achieving \textit{controllable} gesture synthesis through the use of \textit{modality guidance and word-excitation guidance} (discussed in Sec. 3.3).
% %
% We do so in a framework that performs not only \textit{monadic} co-speech generation, but also \textit{two-person} conversational gesture synthesis.
% %
% % %
% % Also important is the fact that we do so not only for the monadic setting, but also for the dyadic (two-person conversation) setting.
% %
% %For more details, we refer the reviewer to Sec. 3.3.

% % 
% % 
% % while the motion is encoded as small chunks, the decoder decodes a collection of chunked encodings together. 

% %
% % This is crucial for providing temporally consistent motion.
% %
% % It is also noteworthy that our auto-encoder is trained to remove jittering artifacts that originate due to the noisy hand motions of the BEAT dataset.
% \par
% \noindent \textbf{On Semantic Consistency [\Rb]:} 
% %As we show in dddd 
% Our method can generate semantically meaningful gestures(03:16-03:36 in Suppl. video), thanks to the proposed Word Excitation Guidance (WEG).
% % Our method produces more semantically coherent gestures compared to the state-of-the-art methods by employing word-excitation guidance.  
% %
% This guidance objective encourages the denoising process to sample gestures that produce more pronounced attention features for the user-selected words.
% %selected by the user.
% %
% %
% % It is worth noting that the term ``semantic coherence/consistence'' has been established rather vaguely in the conversation analysis literature as many gestures can be conceivably semantically coherent, and this differs from speaker to speaker. 
% %
% While quantitatively evaluating such semantic coherence is challenging, we conducted the following ablation to analyze the effect of WEG on semantic coherence.
% %
% First, we trained a binary classifier that classifies $1$s motions of the BEAT dataset into either beat gesture, or semantic gesture type (based on the GT labels).
% %an analysis by training a binary classifier to categorize model predictions into either beat gestures or semantic gestures, which include iconic, metaphoric, and deictic types.
% % 
% % 
% %The classifier was trained on 1-second gesture sequences for the binary classification of semantic and beat gestures. 
% This classifier is then used as an oracle to compute the recall of our generated motions for semantic class predictions.
% %
% Specifically, we extract the speech and text for the sentence in which a semantic gesture has been labeled in dataset.
% %
% These are then input to ConvoFusion to generate the corresponding gestures, with and without WEG.
% %
% For the case of WEG, we focus on the exact words wherein the semantic gesture occurs in the sentence.%use the exact phrase from the ground-truth label.
% % we applied the classifier to our synthesized gestures, both with and without WEG, specifically focusing on points in the BEAT dataset where semantic gestures occur.
% % 
% % That means, first we perform gesture synthesis for the part of text/speech that has semantic gesture type annotated and we do this both with WEG and without it. When using WEG, we focus on words that are annotated corresponding to a semantic gesture. Secondly, we run our trained classifier on both WEG and non-WEG predictions and compare results.
% % 
% % In doing so, the goal is to calculate the recall for semantic class predictions on the motions associated with a semantic gesture type. 
% % 
% We observe that the recall for semantic labels \textit{without WEG} is \underline{0.34}.
% %
% However, when WEG was employed, this recall increased to \underline{0.40}, \textit{indicating that the use of WEG indeed enhances semantic coherence in predictions}.
% %
% We will add this analysis to the revised draft.
% % We observed that, without WEG, the recall for the semantic class was \underline{0.34}.
% % 
% % 
% % It is worth noting that which specific phrases elicit semantic gestures is still an open area of research, as it varies across identities, cultures and situations.
% % %
% % %
% % WEG lets the user control such generation and is, naturally, subject to the presence of such associated gestures in the dataset.

% \par
% \noindent \textbf{The new dataset is small-scale [\Rr]:} 
% The proposed DnD dataset consists of $6$ hours of mocap data comprising of $5$ persons in the scene.
% %
% In total, we have 2.7M poses along with synchronized, per-person audio tracks and text transcripts.
% %
% The proposed dataset addresses a different aspect of human gestures, \textit{i.e.} group conversations, which is a sparsely researched setting.
% %
% This makes our dataset complementary to the existing monadic gesture datasets like BEAT.
% %
% Indeed, we find that jointly using the two datasets, as done in ConvoFusion using modality-dropout, brings the best of both worlds together and prevents such overfitting (Suppl. Sec. 4.2).
% %
% We also request the reviewer to revisit our Suppl. video wherein we show the GT and synthesized motions side-by-side (03:54-05:54).
% %
% Our results are visibly different from the GT, which further proves there is no overfitting.
% %and the same is also captured in the multimodality metric .
% %%
% % Moreover, as mentioned in implementation details (supplementary document section 4.2), we use BEAT and our introduced dataset jointly to train our framework even if they differ in the types of annotations they contain (BEAT does not contain two-person annotations related to dyadic settings)
% % % 
% % This is only possible thanks to modality dropout strategy (which we introduce in Sec 3.3) by turning off dyadic conditioning training only for BEAT training examples while also leveraging the larger dataset size of BEAT.
% % 
% % 
% \par
% \noindent \textbf{Does the dataset capture gestures exhibited in daily conversations?%Relation of Gestures in dataset to daily conversations 
% [\Rb]:} 
% % 
% Finding a capture setting that elicits high density of meaningful, semantic gestures is indeed a challenging task.
% %
% These considerations lead us to capture the participants in a role-playing setting as they need to describe an imaginary world to each other, thereby leading to a high density of semantic gestures.
% %
% The setting also offers a clear intrinsic reward to the participants (of winning the game).
% %
% As we show in the video (02:03-02:35, 05:21-05:54, 08:12-09:20, 10:23-10:56), the gestures in our dataset are similar to the ones appearing in daily conversation because participants are simply discussing a game plan or their next steps in certain situations using language that is colloquially used in conversations. 
% % 
% % Interestingly, the most relevant gestures to the game setting are pointing gestures (participants usually point to objects on table) which are considered deictic gestures, which happen frequently in normal conversations.
% % 
% We highlight that the proposed dataset is recorded in a markerless motion capture setup which it keeps the group conversation natural without restrictions of a capture suite or markers, thereby reducing the Observer's Paradox.
% %because movements are not restricted by clothing, which is usually the case with conventional capture technology.
% % 
% Finally, the subjects are familiar with each other (esp. in the DnD setting) which further helps in more natural conversations.
% %as possible during the recording.
% % \IK{ The setup also includes 3D hand annotations which is difficult to obtain in such a group setting using conventional capture technology. Naturally, our setup makes it easier for the subjects to perform natural daily conversations during recording. The subjects are familiar with each other, and they have also been instructed to converse as natural as possible during the recording.
% % Please also mention the difficulty of bringing multi-hours recording of 5 unique individuals for a speech gesture dataset that exhibit dense semantically meaningful gestures in the conversation.}
% % By roleplaying, we don't mean that participants perform certain specific gestures related to their characters
% \par
% \noindent\textbf{Paper Writing and Abbreviations [\Rr]:}
% We thank the reviewer for pointing to it.
% %
% We will elaborate the motivation appropriately in the introduction which, we reiterate, is \textit{controllable gesture synthesis} and \textit{generalization to monadic and dyadic settings} within a unified approach.
% % 
% Concerning the notations, we will add a table of notations in the revised draft to improve clarity and readability.
% % Moreover, our work contains large number of mathematical notations to explain 3-4 main working parts of our method. and this is reflected in the figures and method section.
% % % 
% % We promise to reduce abbreviations and notations as much as we can. Lastly, we will also add a table for all notations and abbreviations in the supplementary document for ease of reference.
% % 
% % 
% %%%%%%%%% REFERENCES
% \vspace{-0.8em}
% {
%     \small
%     \bibliographystyle{ieeenat_fullname}
%     \bibliography{references}
% }

% \end{document}

